Issue Tracking Ecosystems: Context and Best Practices

Issue Tracking Systems (ITSs), such as GitHub and Jira, are popular tools that support Software Engineering (SE) organisations through the management of ``issues'', which represent different SE artefacts such as requirements, development tasks, and maintenance items. ITSs also support internal linking between issues, and external linking to other tools and information sources. This provides SE organisations key forms of documentation, including forwards and backwards traceability (e.g., Feature Requests linked to sprint releases and code commits linked to Bug Reports). An Issue Tracking Ecosystem (ITE) is the aggregate of the central ITS and the related SE artefacts, stakeholders, and processes -- with an emphasis on how these contextual factors interact with the ITS. The quality of ITEs is central to the success of these organisations and their software products. There are challenges, however, within ITEs, including complex networks of interlinked artefacts and diverse workflows. While ITSs have been the subject of study in SE research for decades, ITEs as a whole need further exploration. In this thesis, I undertake the challenge of understanding ITEs at a broader level, addressing these questions regarding complexity and diversity. I interviewed practitioners and performed archival analysis on a diverse set of ITSs. These analyses revealed the context-dependent nature of ITE problems, highlighting the need for context-specific ITE research. While previous work has produced many solutions to specific ITS problems, these solutions are not consistently framed in a context-rich and comparable way, leading to a desire for more aligned solutions across research and practice. To address this emergent information and lack of alignment, I created the Best Practice Ontology for ITEs. <... truncated due to arXiv abstract character limit ...>

==> 5_backmatter/declaration.tex <==

\cleardoubleevenpage        % Start on the right-hand side (in a book)
\thispagestyle{empty}       % Remove page number

\vspace*{0.3\textheight}    % Add vertical space
\noindent\Large\textbf{Eidesstattliche Erkl{\"a}rung:}
\normalsize                 % Change font size

\vspace{5mm}                % Add vertical space

\noindent                   % No indent on next paragraph start
Hiermit versichere ich an Eides statt, die vorliegende Dissertationsschrift selbst verfasst und keine anderen als die angegebenen Hilfsmittel und Quellen benutzt zu haben.
Sofern im Zuge der Erstellung der vorliegenden Dissertationsschrift generative Künstliche Intelligenz (gKI) basierte elektronische Hilfsmittel verwendet wurden, versichere ich, dass meine eigene Leistung im Vordergrund stand und dass eine vollständige Dokumentation aller verwendeten Hilfsmittel gemäß der Guten wissenschaftlichen Praxis vorliegt. Ich trage die Verantwortung für eventuell durch die gKI generierte fehlerhafte oder verzerrte Inhalte, fehlerhafte Referenzen, Verstöße gegen das Datenschutz- und Urheberrecht oder Plagiate.
\vspace{5mm}                % Add vertical space

\noindent                   % No indent on next paragraph start
Ich versichere, dass dieses gebundene Exemplar der Dissertation und das in elektronischer Form
eingereichte Dissertationsexemplar (über den Docata-Upload) und das bei der Fakultät
(zuständiges Studienbüro bzw. Promotionsbüro Physik) zur Archivierung eingereichte gedruckte
gebundene Exemplar der Dissertationsschrift identisch sind.

\vspace{4cm}                % Add vertical space

\noindent Hamburg, den \hdashrule{3cm}{1pt}{1pt} \hspace{1cm} \hdashrule{7.5cm}{1pt}{1pt}

\hspace{6.5cm} Lloyd Montgomery

